Chimera: A Lossless Decoding Method for Accelerating Large Language Models Inference by Fusing all Tokens

Large language models (LLMs) have demonstrated remarkable capabilities across various tasks. However, their widespread application is hindered by the resource-intensive decoding process. To address this challenge, current approaches have incorporated additional decoding heads to enable parallel prediction of multiple subsequent tokens, thereby achieving inference acceleration. Nevertheless, the accuracy of these decoding heads falls short of the auto-regressive decoding approach. In light of these limitations, we propose Chimera, a novel framework specifically designed for speculative sampling. Within this framework, we introduce a lightweight draft model that effectively utilizes previously generated tokens to predict subsequent words. To ensure both accuracy and efficiency, we present two strategies within the lightweight draft model. Firstly, we focus on capturing short-range dependencies at the bottom layer. Secondly, we leverage the readily available representations from the original LLM.Through empirical evaluation on the Vicuna and LlaMA-2 series, Chimera demonstrates impressive results, achieving an average latency speedup ratio of 2.7x compared to the vanilla auto-regressive decoding approach. This highlights the potential of our proposed framework in significantly improving the efficiency of large language models during the decoding process.

==> latex/sections/abstract.tex <==
\begin{abstract}
%Large language models (LLMs) have demonstrate impressive capacity in various tasks. However, the costly decoding process is hinder its wide application. 
%their text generation process is costly and slow. This inefficiency stems from the nature of autoregressive decoding, where each token generation requires a forward pass and access to the entire parameter set of the LLM, which can reach hundreds of billions or even trillions of parameters. This leads to memory limitations in autoregressive decoding.
%One approach to accelerate autoregressive decoding is speculative decoding. This technique employs a smaller draft model to guess the next γ token based on standard autoregressive generation. Subsequently, the original LLM validates these guessed tokens, requiring only one forward pass for validation. If the draft model accurately predicts α tokens, the original LLM's single forward pass can generate α+1 tokens. However, current speculative decoding still faces several issues. First, the quality of drafts generated by small models is low, limiting the effectiveness of acceleration. Second, placing the small model on multiple GPUs for draft generation increases memory access and GPU communication time.

%Therefore, this paper proposes a universal framework called Chimera to accelerate the inference process. It combines the rich semantic information from the high-level representations in the output of the original LLM with the shallow semantic information of the newly generated tokens to predict drafts. This enhances the quality of draft generation. Additionally, as a lightweight plugin, Chimera can be loaded on the same GPU as the large model, reducing memory access and communication time. In the inference process of Chimera, the framework first collects the hidden layer output of the last transformer layer in the original model and the next token being inferred. It queries the trigram of the inference token and fuses it with the original hidden output through a small number of transformer layers to predict the next token's original hidden layer output. The draft can be obtained by passing the hidden layer output through an MLP head. Repeating this process yields drafts containing multiple tokens. Our strategy has two distinct advantages: (1) theoretically no limit on the length of generated drafts (2) our method only requires a small number of transformer layers and MLP layers, making it very lightweight. We conducted extensive experiments to demonstrate significant improvements achieved by applying our inference acceleration framework.
Large language models (LLMs) have demonstrated remarkable capabilities across various tasks. 
However, their widespread application is hindered by the resource-intensive decoding process. 
To address this challenge, current approaches have incorporated additional decoding heads to enable parallel prediction of multiple subsequent tokens, thereby achieving inference acceleration. 
Nevertheless, the accuracy of these decoding heads falls short of the auto-regressive decoding approach. 
In light of these limitations, we propose Chimera, a novel framework specifically designed for speculative sampling. Within this framework, we introduce a lightweight draft model that effectively utilizes previously generated tokens to predict subsequent words. 
To ensure both accuracy and efficiency, we present two strategies within the lightweight draft model. 
Firstly, we focus on capturing short-range dependencies at the bottom layer. 
Secondly, we leverage the readily available representations from the original LLM. 
Through empirical evaluation on the Vicuna and LlaMA-2-chat series, Chimera demonstrates impressive results, achieving an average latency speedup ratio of 2.7x compared to the vanilla auto-regressive decoding approach. 
This highlights the potential of our proposed framework in significantly improving the efficiency of large language models during the decoding process.
% Large language models (LLMs) have demonstrated impressive capacity in various tasks. 
% However, the costly decoding process hinders its wide application.
% Current methods added extra decoding heads to predict multiple subsequent tokens in parallel, achieving inference acceleration.
% However, the accuracies of decoding heads are lower than the auto-regressive decoding head. 
% We introduced Chimera, a novel framework designed for speculative sampling. 
% We propose a lightweight draft model that effectively leverages previously generated tokens to predict subsequent words. 
%Key strategies include capturing short-range dependencies through a trigram encoder and utilizing the full context provided by the original language model.
% We propose two strategies within the lightweight draft model to ensure accuracy and efficiency, i.e., capturing short-range dependencies at the bottom layer and taking advantage of readily available representation from the original LLM. 
% On the Vicuna and LlaMA-2 series, Chimera achieved an average latency speedup ratio of 2.7x compared to vanilla auto-regressive decoding.
\end{abstract}

